Min-Cost Flow Routing for Evidence Assembly in Long Multimodal Documents

Answering questions about long multimodal documents requires distributing a fixed evidence budget across relevant facets in text, tables, figures, and slides while avoiding near-duplicates. We present \flowreader, which formulates evidence selection as a single minimum-cost flow problem with capacity limits over a multimodal content graph. Spectral decomposition identifies latent aspects of query-relevant content and allocates the budget among them in proportion to their spectral energy. These capacity limits enforce aspect coverage during routing without requiring a language-model planning call. Query-conditioned costs prioritize chains of relevant, mutually consistent evidence. Decomposing the optimal flow produces short evidence chains, which a vision-language model reads in parallel and a reasoner reconciles. On VisDoMBench with Qwen3-VL-32B, \flowreader\ achieves the highest macro accuracy ($68.9$), surpassing the strongest prior system by $2.7$ points, leading on three of five subsets and attaining the highest worst-subset accuracy. It uses a measured $17.5$ content nodes per query and maintains its lead at $12.9$. Ablation studies with a fixed graph, scorer, reader, and judge show that cost design drives accuracy, capacity limits preserve it while using about three-quarters of the reader tokens required by shortest-path routing without these limits on the same network, and spectral aspects align with LLM-generated sub-questions without a planning call.

==> Sections/limitations.tex <==
\section{Limitations}
The primary advantage of \flowreader\ is improved evidence efficiency, not higher accuracy under a loose budget. The shortest-path approach on the same graph achieves comparable accuracy at the same node budget ($p = 0.86$) but requires reading the evidence $49.4$ times, compared with $23.3$ for \flowreader. Similarly, min-cost flow, relevance ranking, and PPR-diffused top-$k$ methods place an answer-bearing node before a reader at similar rates ($66.9$, $67.0$, and $66.9$ percent, respectively), suggesting the benefit lies in budget allocation. The chain selector constitutes a minor component: greedy selection at a matched read cap performs within the margin of replicator dynamics ($0.3$ points, $p = 0.68$). Results are based on a single benchmark with one reader backbone and one judge. The baseline's $30$ to $40$ node budget is derived from its stated configuration rather than direct measurement. The system is not adaptive: it caps demand at its upper bound for nearly every query, and it finalizes all routing and selection decisions before reading any evidence. The potential benefit of a second solve informed by the first remains undetermined.

==> Sections/setup.tex <==
\section{Experimental Setup}
\subsection{Benchmark}
\subsection{Baselines}
\subsection{Why sizteen chains}

